Guaranteed Discovery of Control-Endogenous Latent States with Multi-Step Inverse Models

In many sequential decision-making tasks, the agent is not able to model the full complexity of the world, which consists of multitudes of relevant and irrelevant information. For example, a person walking along a city street who tries to model all aspects of the world would quickly be overwhelmed by a multitude of shops, cars, and people moving in and out of view, each following their own complex and inscrutable dynamics. Is it possible to turn the agent's firehose of sensory information into a minimal latent state that is both necessary and sufficient for an agent to successfully act in the world? We formulate this question concretely, and propose the Agent Control-Endogenous State Discovery algorithm (AC-State), which has theoretical guarantees and is practically demonstrated to discover the minimal control-endogenous latent state which contains all of the information necessary for controlling the agent, while fully discarding all irrelevant information. This algorithm consists of a multi-step inverse model (predicting actions from distant observations) with an information bottleneck. AC-State enables localization, exploration, and navigation without reward or demonstrations. We demonstrate the discovery of the control-endogenous latent state in three domains: localizing a robot arm with distractions (e.g., changing lighting conditions and background), exploring a maze alongside other agents, and navigating in the Matterport house simulator.

==> extra.tex <==
%auto-ignore

Simple Algorithm: 

\begin{itemize}
    \item We use any roll-in policy.  
    \item We use a roll-out policy which only depends on the endogenous state.  For simple algorithm this is a random roll-out policy.  
    \item We train genik objective on all roll-outs up to a fixed limit K (which we advise to set to the longest shortest path in endogenous-graph).  
    \item $\mathcal{L} = \mathcal{L}_{inv} + \mathcal{L}_{ib}$.  
\end{itemize}

More General Algorithm: 

\begin{itemize}
    \item We use any roll-in policy.  
    \item Use current endogenous state to construct a plan to reach a goal state with an expected $K$ steps.  
    \item We follow the plan for $K$ steps and take a single random action during the rollout.  
    \item We train genik only on random actions.  
\end{itemize}

Write up as actual algorithm blocks.  The IB objective is flexible $min_\phi MI(x, \phi(x))$ but right now we accomplish it with: (1) variational gaussian information bottleneck, (2) VQ discretization, (3) architectural inductive biases.  

\begin{figure}
    \centering
    \subfloat[][VAE\\(Theory Worst-Case)]{\includegraphics[width=0.3\linewidth]{figures/robot_confusion/vae_theory.png}}
    \subfloat[][Inverse\\(Theory Worst-Case)]{\includegraphics[width=0.3\linewidth]{figures/robot_confusion/inverse_theory.png}}
    \subfloat[AC-State\\(Theory Worst Case)]{\includegraphics[width=0.3\linewidth]{figures/robot_confusion/genik_theory.png}}\\
    \subfloat[VAE\\(Empirical)]{ \includegraphics[width=0.3\linewidth]{figures/robot_confusion/vae.png}}
    \subfloat[Inverse\\(Empirical)]{\includegraphics[width=0.3\linewidth]{figures/robot_confusion/inverse.png}}
    \subfloat[AC-State\\(Empirical)]{\includegraphics[width=0.3\linewidth]{figures/robot_confusion/genik.png}}
    \caption{ }
    \label{fig:my_label}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/hard_reset/heatmap_random_rollout.png}
    \includegraphics[width=0.9\linewidth]{figures/hard_reset/heatmap_goal_seek.png}
    \caption{Random Rollout (top) and using AC-State to plan to reach rarely visited latent states (bottom) in an environment where one third of the actions reset the agent's position to the top left corner.  A random policy fails to explore the environment whereas using AC-State is able to efficiently explore.  }
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.29\linewidth]{figures/robot/Input.png}
    \includegraphics[width=0.29\linewidth]{figures/robot/Latent.png}
    \includegraphics[width=0.40\linewidth]{figures/designer_figs/heatmap_designer.png}
    \label{fig:MFL}
    \caption{Robot experiment.  The algorithm learns the latent space despite distractions.  It is interesting to note that the distractions (marked in red) are greyed out in the latent image.  Example of Observation Image.  Contains several distractions like TV, drinking birds, flashing lights etc. Latent state image decoder learned by passing the detached latent state as input and trying to minimize error between the input and output images.Latent state image decoder learned by passing the detached latent state as input and trying to minimize error between the input and output images.  We show the latent state discovery on data-collected from the robot, along with the theoretical worst case for an optimal model.  The autoencoder (VAE) gives no effective theoretical guarantee in the presence of overwhelming visual distractors and indeed fails to discover the controllable latent state in practice.  The one-step inverse model performs better but fails to correctly discover \textit{long range dependencies} both in theory and in practice.  AC-state has perfect theoretical discovery and nearly perfect discovery in practice. }
\end{figure}

\begin{figure}
    \centering
    \hfill
    \fbox{\includegraphics[width=1.0\linewidth,height=0.33\linewidth]{figures/mazes/spiral/annotated-maze-spiral.png}}
    \hfill
    \includegraphics[width=1.0\linewidth,height=0.025\linewidth]{figures/mazes/spacer.png}
    \hfill
    \fbox{\includegraphics[width=1.0\linewidth,height=0.33\linewidth]{figures/mazes/4room/annotated-maze.png}}
    \hfill
    \subfloat[Image seen by Camera \\\\ Nine agents moving in different mazes.  Only one {\bf agent is controlled}  (yellow) by the algorithm.  The rest are {\bf distractions} (blue).  It’s important to note that the agent {\bf does not} see the yellow and blue coloring.] {\includegraphics[width=0.3\linewidth,height=0.001\linewidth]{figures/mazes/spacer.png}}
    \hspace{.5cm}
    \subfloat[True dynamics of the agent \\\\ Each node (red square) represents a position that the agent can move to.  The green lines represent the paths that the agent can take between nodes. ]{{\includegraphics[width=0.3\linewidth,height=0.001\linewidth]{figures/mazes/spacer.png}}}
    \hspace{.5cm}
    \subfloat[Learned dynamics visualization \\\\ The algorithm can perfectly learn the underlying dynamics of the controlled agent, even in the presence of distracting stimuli.  This visualization uses a graph-plotting software to plot states as nodes and transitions as edges (the exact position of the nodes is arbitrary).  ]{{\includegraphics[width=0.3\linewidth,height=0.001\linewidth]{figures/mazes/spacer.png} }}%
    \hspace{.5cm}
    \hfill
    \label{fig:MFL}
    \caption{Maze experiment}
\end{figure}

 %attempting to control the robot with Denavit-Hartenberg conventions or Brockett's exponential map.  %For a robot arm planar manipulation problem, for example,   The arm and the objects' physical orientation and characteristics describe the dynamics\footnote{By the dynamics of a system, we mean a (mathematical) representation of the behavioral evolution of the system.}. 
% Our claim in this report

%The kinematics and kinetics of physical phenomena can be described by a set of generalized coordinates, or kinodynamic parameterizations that govern the forces, momenta, position and velocity of an agent or system. In large state spaces, however, explicitly modeling these causal parameters become difficult, particularly in the presence of kinodynamic constraints in the state space. 

%For example, consider a Newtonian setting concerned with abstracting a set of billiard balls' motion on a table. In generalized coordinates, the balls' masses, physical locations (described by their respective positions and velocities\footnote{Essentially, those properties that affect its kinetics and kinematics.}) describe the balls' dynamics
% \footnote{Essentially, those properties that affect its kinetics and kinematics.}

%%LM 06/04: Compliance in robot manipulators is a necessity for articulated manipulation of structures, in particular those with nonlinear geometry. Imposing forces and torques on the tool frame of the robot to solve a precise positioning problem typically introduces links deformation and flexure, internal sensors' drive backlash such that computed homogeneous transformations lack numerical precision to realize effective control. In tasks where passive compliance is a requirement, learning the latent state of the robot is beneficial for accuracy in positioning-based manipulation and locomotion tasks.
\subsection{Stochastic Controllable Latent Dynamics}

In the proof for Theorem~\ref{thm:phi_star_coarsest} we assumed that the controllable latent dynamics are deterministic.  This is used to establish the notion of reachability in a binary sense (a state is either considered reachable or not). In the absence of this assumption, the \textit{AC-State} algorithm may still work on a reasonable class of problems with stochastic controllable latent dynamics (in particular, those which are nearly-deterministic).  Achieving a general solution on all stochastic problems may require an adaptation of the \textit{AC-State} algorithm.  

%For an agent that is interacting with an environment, discovering a latent state and its associated transition structure could enable the agent to localize itself within an environment, navigate and explore in that environment, facilitate communication with other agents in the loop, and could simplify debugging by system developers.  Localization is the process of mapping sensory inputs into the latent state, enabling all other capabilities. Planning to navigate to a goal can be accomplished via several algorithms such as finding the shortest path, using dynamic programming, or Monte Carlo sampling procedures. Planned exploration is a critical ability in situations (such as climbing up a steep cliff) where random exploration has exponentially small odds of success. Generally, some tasks (such as a robot vacuum) are about coverage of the controllable state space. A good latent state is naturally parsimonious providing a natural method for humans to specify goals for an agent or for the agent to describe its situation. A latent state representation can also be compared with the basic physical interpretation of the world to discover discrepancies, which can then be debugged by a system developer. \dipendra{this paragraph doesn't flow. Lines constantly change topic that is being discussed from localization, exploration, to suddenly about communication}


%\cite[Prop4]{arxivPaper}
%\dipendra{while this is true, the real magic is that the AC-State objective is such that it wont suffer from this constriction. This part needs to be emphasized as it is our key novelty}

%The former is more straightforward, while the latter is necessary in situations where random exploration works rarely


    %\caption{Robot results (should have algorithm figure integrated).  Robot experiment.  The algorithm learns the latent space despite distractions.  It is interesting to note that the distractions (marked in red) are greyed out in the latent image.  Example of Observation Image.  Contains several distractions like TV, drinking birds, flashing lights etc. Latent state image decoder learned by passing the detached latent state as input and trying to minimize error between the input and output images.Latent state image decoder learned by passing the detached latent state as input and trying to minimize error between the input and output images.  We show the latent state discovery on data-collected from the robot, along with the theoretical worst case for an optimal model.  The autoencoder (VAE) gives no effective theoretical guarantee in the presence of overwhelming visual distractors and indeed fails to discover the controllable latent state in practice.  The one-step inverse model performs better but fails to correctly discover \textit{long range dependencies} both in theory and in practice.  AC-state has perfect theoretical discovery and nearly perfect discovery in practice.  }
A good latent state is naturally parsimonious providing a natural method for humans to specify goals for an agent or for the agent to describe its situation. 
\textbf{Failure of Contrastive Learning: } 

\textbf{Failure of Bisimulation: }

\textbf{Failure of Autoencoding: } 

\textbf{Failure of Modeling of Transition Dynamics: } 

\textbf{Failure of Inverse Dynamics: }

\textbf{Failure of BYOL: }

\textbf{Failure of Reward-Based Approaches: }

\textbf{: } 

%Classical approaches such as simultaneous localization and mapping (SLAM) and before that Kalman Filters provide techniques for accomplishing this task specialized to individual sensors.  
%Deep learning has been used for latent state learning, but no algorithm has been proposed which provably discards exogenous information.  

An agent interacting with the world must map high-dimensional sensory inputs such as a megapixel camera into actions.  These high-dimensional inputs are characterized by systemic structural distractions from lighting, wind, ancillary objects, and other sources.  Winnowing this information source down to a parsimonious latent state capturing \emph{only} the agent-system interaction dynamics enables tasks such as localization, navigation, and debugging for applications such as robotic control, navigating cars, and even dialog systems. 


==> finitesample_proof.tex <==
%auto-ignore

\subsection{Finite-Sample Analysis for Episodic Setting}
\label{sec:finitesample}

In this section, we consider episodic setting but allow the transition to be stochastic as long as certain margin conditions hold.

Let $\omega$ be the distribution used to collect episodes. In particular, $\omega(x_t, a_t, x_h)$ denotes marginal distribution over $(x_t, a_t, x_h)$ for $t, h \in [H+1]$ and $t < h$. We make the following assumption on the data collection distribution $\omega$:

\begin{assumption}\label{assum:data-collection} The data collection distribution $\omega$ is \emph{exogenous-free}, i.e., we have 
\begin{equation}
    \omega(x_t, a_t) = \omega(x_t) \omega(a_t \mid \edo(x_t)), \qquad t \in [H], x_t \in \Xcal_t, a_t \in \Acal.
\end{equation}
\end{assumption}

We use a modified form of \selfstate algorithm shown in Algorithm~\ref{alg:modified-episodic-alg}. The algorithm assumes access to two function classes $\Phi_N$ and $\Pcal$, and a failure probability hyperparameter $\delta \in (0, 1)$. The function class $\Phi_N = \{\phi: \Xcal \rightarrow [N]\}$ where $N \in \NN$ consists of a set of encoders that map an observation to one of the $N$ latent states. The other function class $\Pcal = \{p: [N]^2 \times [H]^2 \rightarrow \Delta(\Acal) \}$, models classifier that given a pair of latent state observed at two different time steps, output probability over actions. We define $\Fcal = \Pcal \circ \Phi_N = \{f: x, x' \mapsto p(\cdot \mid \phi(x), \phi(x') \mid p \in \Pcal, \phi \in \Phi_N\}$. We assume that $\Fcal$ is finite for simplicity and our sample complexity results with scale as $\ln|\Fcal|$. 

The algorithm collects a list $\Dcal$ of tuples $(x, a, x', t, h)$ using the data generation process (line~\ref{line:data-generation-starts}-\ref{line:data-generation-end}). The algorithm then solves the \selfstate optimization $\Dcal$ and obtains the empirical risk minimizer (ERM) solution $\hat{f}$ in line~\ref{line:erm-solution-episodic}. The latent state decoder $\hat{\phi}$ is the decoder in $\hat{f}$. This is used to estimate the latent dynamics $\hat{T}$ using count-based estimation (line~\ref{line:latent-dynamics-estimation}). The algorithm returns the latent decoder and the learned dynamics.

\begin{algorithm}
\caption{Episodic version of $\selfstate$. \\Input: function classes $\Phi_N$ and $\Pcal$, and hyperparameter $\delta \in (0, 1)$.}
\label{alg:modified-episodic-alg}
\begin{algorithmic}[1]
\State $\Dcal = \emptyset$ 
\For{$n$ times}\label{line:data-generation-starts}
\State Sample $h$ uniformly from $\{2, 3, \cdots, H+1\}$ and $t$ uniformly from $[h-1]$
\State Sample an episode $(x_1, a_1, x_2, a_2, \cdots, x_H, a_H, x_{H+1})$ from $\omega$
\State $\Dcal \leftarrow \Dcal \cup \{(x_t, a_t, x_h, t, h)\}$
\EndFor\label{line:data-generation-end}
\State Solve the $\selfstate$ optimization problem: \label{line:erm-solution-episodic}
\begin{equation}\label{eqn:erm-finite-sample}
    \hat{f} := \hat{p}, \hat{\phi} = \arg\max_{p \in \Pcal, \phi \in \Phi_N} \sum_{(x, a, x', t, h) \in \Dcal} \ln p(a \mid \phi(x), \phi(x'), t, h)
\end{equation}
\State Estimate latent dynamics $\hat{T}: [N] \times \Acal \rightarrow \Delta([N])$ by applying decoder $\hat{\phi}$ on $\Dcal$.\label{line:latent-dynamics-estimation}
\State return $\hat{\phi}$ and $\hat{T}$.
\end{algorithmic}
\end{algorithm}


\paragraph{Notations.} We will use $\PP(\xi_t)$ to denote the distribution over exogenous state $\xi$ at time step $t \in [H+1]$. For $1 \le t < h \le H+1$, w define $\PP(\xi_h \mid \xi_t)$ as the conditional probability over exogenous state at time step $h$ given its value at time step $t$. We will also use a shorthand $q(x)$ to denote $q(x \mid \edo(x), \exo(x))$ probability of generating observation $x$ given the endogenous state and exogenous state of $x$.


Similar to earlier section, assumption~\ref{assum:data-collection} implies the following factorization results.
\begin{lemma}\label{lem:state-factorization} For any $t \in [H+1]$, the marginal distribution $\omega(s_t, \xi_t)$ factorizes as:
\begin{equation*}
    \omega(s_t, \xi_t) = \omega(s_t)\omega(\xi_t).
\end{equation*}
\end{lemma}
\begin{proof} Proof is by induction on $t$. In base case, $(s_1, \xi_1)$ is sampled from a start state distribution $\mu$ which factorizes as follows:
\begin{equation*}
    \mu(s_1, \xi_1) = \mu(s_1)\mu_\xi(\xi_1).
\end{equation*}
As $\omega(s_1) = \mu(s_1)$ and $\omega(\xi_1) = \mu_\xi(\xi_1)$, therefore, base case holds. Now suppose the factorization holds for some $t < H+1$. Then we have:
\begin{align*}
    \omega(s_{t+1}, \xi_{t+1}) &= \EE_{(s_t, \xi_t, a_t) \sim \omega}\left[\PP(s_{t+1}, \xi_{t+1} \mid s_t, \xi_t, a_t)\right]\\
    &= \EE_{(s_t, \xi_t, a_t) \sim \omega}\left[T(s_{t+1}, \mid s_t, a_t) \PP(\xi_{t+1} \mid \xi_t)\right]\\
    &= \EE_{(s_t, \xi_t) \sim \omega, a_t \sim \omega(\cdot \mid s_t)}\left[T(s_{t+1}, \mid s_t, a_t) \PP(\xi_{t+1} \mid \xi_t)\right]\\
    &= \EE_{s_t \sim \omega, \xi_t \sim \omega, a_t \sim \omega(\cdot \mid s_t)}\left[T(s_{t+1}, \mid s_t, a_t) \PP(\xi_{t+1} \mid \xi_t)\right]\\
    &= \EE_{s_t \sim \omega, a_t \sim \omega(\cdot \mid s_t)}\left[T(s_{t+1}, \mid s_t, a_t) \right]\EE_{\xi_t \sim \omega}\left[\PP(\xi_{t+1} \mid \xi_t)\right].
\end{align*}
By marginalizing out $s_{t+1}$ and $\xi_{t+1}$, we can verify that $\omega(s_{t+1}) = \EE_{s_t \sim \omega, a_t \sim \omega(\cdot \mid s_t)}$ and $\omega(\xi_{t+1}) = \EE_{\xi_t \sim \omega}\left[\PP(\xi_{t+1} \mid \xi_t)\right]$, therefore, we have: $\omega(s_{t+1}, \xi_{t+1}) = \omega(s_{t+1})\omega(\xi_{t+1})$. 
\end{proof}


\begin{lemma}\label{lem:data-distribution-factorization} For any $1 \le t < h \le H+1$, and $x, x' \in \Xcal, a \in \Acal$, we have:
\begin{equation*}
    \omega(x_t, a_t, x_h) = q(x_t) q(x_h) \omega(\edo(x_t), a_t, \edo(x_h)) \PP(\exo(x_h) \mid \exo(x_t))
\end{equation*}
\end{lemma}
\begin{proof} Proof is by induction. Fix $h \in [H+1]$. We will show that the result holds for all $t < h$. Let $s_h = \edo(x_h), \xi_h = \exo(x_h), s_t = \edo(x_t)$ and $\xi_t = \exo(x_t)$. We first consider the base case ($t=h-1)$. 
\begin{align*}
    & \omega(x_{h-1}, a_{h-1}, x_h) \\
    &= \omega(x_{h-1}, a_{h-1}) T(x_h \mid x_{h-1}, a_{h-1})\\
    &= q(x_h) \omega(x_{h-1}, a_{h-1}) T(s_h \mid s_{h-1}, a_{h-1}) \PP(\xi_h \mid \xi_{h-1})\\
    &= q(x_h) \omega(x_{h-1})\omega(a_{h-1} \mid s_{h-1}) T(s_h \mid s_{h-1}, a_{h-1}) \PP(\xi_h \mid \xi_{h-1})\\
    &= q(x_h) q(x_{h-1}) \left\{\omega(s_{h-1}) \omega(a_{h-1} \mid s_{h-1}) T(s_h \mid s_{h-1}, a_{h-1})\right\} \left\{\PP(\xi_h \mid \xi_{h-1})\omega(\xi_{h-1})\right\}\\
    &= q(x_h) q(x_{h-1}) \omega(s_{h-1}, a_{h-1}, s_h) \PP(\xi_{h-1}, \xi_h)
\end{align*}

Using Lemma~\ref{lem:state-factorization} we have: 
\begin{align*}
    \omega(x_{h-1}) &= q(x_{h-1}) \omega(s_{h-1}=\edo(x_{h-1}), \xi_{h-1}=\exo(x_{h-1})) \\
    &= q(x_{h-1}) \omega(s_{h-1}=\edo(x_{h-1}))\omega(\xi_{h-1}=\exo(x_{h-1})) = 
\end{align*}

\end{proof}


The dataset $\Dcal$ is used to solve the following optimization problem:


The distribution $D$ over $(t, h, x, a, x')$ is given by:
\begin{equation*}
    D(x, a, x', t, h) = \frac{2}{H(H+1)} \omega(x_t=a, a_t=a, x_h=x')
\end{equation*}
and let the marginal distribution over $(t, h, x, x')$ be denoted as $D(x, x', t, h)$.

\begin{lemma}The Bayes's classifier $f^\star$ satisfies, for all $t, h \in [H+1]$ with $t < h$, and $(x, x') \in {\tt supp}~\omega(x_t, x_h)$, the following:
\begin{equation*}
\forall a \in \Acal, \qquad    f^\star(a \mid x, x', t, h) = \frac{\omega(s_t=\edo(x), a_t=a, s_h=\edo(x'))}{\sum_{a' \in \Acal} \omega(s_t=\edo(x), a_t=a', s_h=\edo(x'))}.
\end{equation*}
\end{lemma}
\begin{proof}
The Bayes classifier $f^\star$ of the problem is given by:
\begin{align*}
    f^\star(a \mid x, x', t, h) &= \PP(a \mid x, x', t, h) \\
    &= \frac{\PP(t, h, x, a, x')}{\sum_{a' \in \Acal} \PP(t, h, x, a', x')}\\
    &= \frac{\PP(x, a, x' \mid t, h)}{\sum_{a' \in \Acal} \PP(x, a', x' \mid t, h)}\\
    &=\frac{\omega(x_t=x, a_t=a, x_h=x')}{\sum_{a' \in \Acal} \omega(x_t=x, a_t=a', x_h=x')}\\
    &= \frac{\omega(x_t=x, a_t=a, x_h=x')}{\sum_{a' \in \Acal} \omega(x_t=x, a_t=a', x_h=x')}\\
    &= \frac{\omega(s_t=\edo(x), a_t=a, s_h=\edo(x'))}{\sum_{a' \in \Acal} \omega(s_t=\edo(x), a_t=a', s_h=\edo(x'))}.
\end{align*}
The first line uses the fact that Bayes's classifier for log-loss is given by the conditional distribution $\PP(a \mid x, x', t, h)$ of the data distribution. The last inequality uses the property of $\omega$ stated in Lemma~\ref{lem:data-distribution-factorization}.
\end{proof}

As the Bayes's classifier $f^\star$ only depends on endogenous state and action, we can define $f^\star(a \mid s, s', t, h)$ as:
\begin{equation*}
    f^\star(a \mid s, s', t, h) = \frac{\omega(s_t=s, a_t=a, s_h=s')}{\sum_{a' \in \Acal} \omega(s_t=s, a_t=a', s_h=s')}
\end{equation*}

\begin{theorem}(Generalization Guarantee) Let $\hat{f}$ be the ERM solution for dataset $\Dcal$ of size $n$ in Equation~\ref{eqn:erm-finite-sample} of Algorithm~\ref{alg:modified-episodic-alg}. Then for any fixed probability $\delta \in (0, 1)$, we have with probability at least $1-\delta$, the following:
\begin{equation*}
    \EE_{(x, x', t, h) \sim D}\left[\TV{\hat{f}(\cdot \mid x, x', t, h) - f^\star(\cdot \mid x, x', t, h)}\right] \le \Delta(n, \delta) :=  \sqrt{\frac{2}{n}\ln\left(\frac{|\Fcal|}{\delta}\right)}
\end{equation*}
\end{theorem}
\paragraph{Remark:} This is a well-known result and we refer interested readers to Appendix E in~\cite{AgarwalKKS20}. The proof immediately follows from using Theorem 21 in~\cite{AgarwalKKS20} by using the fact that samples consist of i.i.d data, and then applying Jensen's inequality for square function.

We will now define a set of distributions that will be helpful for proving the main result.

\paragraph{Coupling distributions.}  We define a forward coupling distribution as:
\begin{equation}\label{eqn:forward-couple-obs}
    P_f(t, h, x, \xtil, x') := \frac{2}{H(H+1)}\omega(x_t=x \mid x_h=x')\omega(x_t=\xtil \mid x_h=x') \omega(x_h=x')
\end{equation}
We similarly define the forward coupling distribution over endogenous state as:
\begin{equation}\label{eqn:forward-couple-state}
    P_f(t, h, s, \stil, s') := \frac{2}{H(H+1)}\omega(s_t=s \mid s_h=s')\omega(s_t=\tilde{s} \mid s_h=s') \omega(s_h=s')
\end{equation}

We also define a backward coupling distribution as:
\begin{equation}\label{eqn:backward-couple-obs}
    P_b(t, h, x, x', \xtil') := \frac{2}{H(H+1)}\omega(x_t=x)\omega(x_h=x' \mid x_t=x)\omega(x_h=\xtil' \mid x_t=x)
\end{equation}
which can be similarly defined over endogenous state as:
\begin{equation}\label{eqn:backward-couple-state}
    P_b(t, h, s, s', \stil') := \frac{2}{H(H+1)}\omega(s_t=s)\omega(s_h=s' \mid s_t=s)\omega(s_h=\stil' \mid s_t=s).
\end{equation}

Before stating the next result, we define a useful quantity. For any $t, h \in [H+1]$ and $t < h$, we have:
\begin{equation}\label{eqn:useful-forward-exo-defn}
    P_f(\xi, \xitil, \xi' \mid t, h) = \PP(\xi_t=\xi \mid \xi_h=\xi')\PP(\xi_t=\xitil \mid \xi_h=\xi') \PP(\xi_h=\xi')
\end{equation}

We can prove the following lemma:
\begin{lemma}(Factorization Lemma). The coupling distributions satisfy:
\begin{equation*}
    P_f(t, h, x, \xtil, x') = q(x) q(\xtil) q(x') P_f(t, h, \edo(x), \edo(\xtil), \edo(x')) P_f(\exo(x), \exo(\xtil), \exo(x') \mid t, h).
\end{equation*}
\end{lemma}
\begin{proof}
We have:
\begin{align*}
    \omega(x_t = x \mid x_h = x') &= \frac{\omega(x_t=x, x_h=x')}{\omega(x_h=x')} \\
    &= q(x) \PP(\xi_t=\exo(x) \mid \xi_h=\exo(x'))\omega(s_t = \edo(x) \mid s_h=\edo(x'))
\end{align*}
We can similarly show
\begin{align*}
    \omega(x_t=\xtil \mid x_h = x') = q(\xtil) \PP(\xi_t=\exo(\xtil) \mid \xi_h=\exo(x'))\omega(s_t = \edo(\xtil) \mid s_h=\edo(x'))
\end{align*}
Lastly, we have $\omega(x_h=x') = q(x') \omega(s_h=x') \PP(\xi_h=\exo(x'))$. Using the definition of $P_f(t, h, x, \xtil, x')$ and the above relations, we get:
\begin{align*}
    P_f(t, h, x, \xtil, x') &= \frac{2}{H(H+1)}q(x) q(\xtil) q(x') \times  \\
&\omega(s_t = \edo(x) \mid s_h=\edo(x'))    \omega(s_t = \edo(\xtil) \mid s_h=\edo(x')) \omega(s_h=x') \times \\
& \PP(\xi_t=\exo(x) \mid \xi_h=\exo(x'))\PP(\xi_t=\exo(\xtil) \mid \xi_h=\exo(x')) \PP(\xi_h=\exo(x'))\\
&= q(x) q(\xtil) q(x') P_f(t, h, \edo(x), \edo(\xtil), \edo(x')) P_f(\exo(x), \exo(\xtil), \exo(x') \mid t, h).
\end{align*}
where the last line uses Equation~\ref{eqn:useful-forward-exo-defn}.
\end{proof}

\paragraph{Margin.} We define a forward $\Gamma_f$ and backward margin $\Gamma_b$ as:
\begin{align}
    \Gamma_f &= \sum_{s, \stil \in \Scal, s \ne \stil}  
   \sum_{1 \le t < h \le H+1} \sum_{s' \in \Scal} P_f(t, h, s, \stil, s') \TV{f^\star(\cdot \mid s, s', t, h) - f^\star(\cdot \mid \stil, s', t, h)}\\
    \Gamma_b &= \min_{s', \stil' \in \Scal, s' \ne \stil'} \sum_{t, h, s} P_b(t, h, s, s', \stil')\|f^\star(\cdot \mid s, s', t, h) - f^\star(\cdot \mid s, \stil', t, h)\|_{TV}
\end{align}

Note that marginal distribution over $(t, h, \tilde{x}, x')$ for $P_f$ is given by $D(t, h, \tilde{x}, x')$ and marginal distribution over $(t, h, x, x')$ for $P_f$ is given by $D(t, h, x, x')$. Similarly, marginal distribution over $(t, h, x, x')$ for $P_b$ is given by $D(t, h, x, x')$ and marginal distribution over $(t, h, x, \tilde{x}')$ is given by $P_b(t, h, x, \tilde{x}')$.


\begin{lemma}(DSM Result.) Fix $\delta \in (0, 1)$. Given $\hat{f} = \hat{p}, \hat{\phi}$ as the ERM solution with $n$ samples, we have with probability at least $1-\delta$ the following: for any two different states $s, \stil \in \Scal$:
\begin{equation*}
  \PP_{x \sim q(\cdot \mid s, \xi), \xtil \sim q(\cdot \mid \stil, \xitil), (\xi, \xitil, \xi') \sim P_f(\cdot, \cdot, \cdot \mid t, h)}\left(\hat{\phi}(x) = \hat{\phi}(\xtil)\right) \le \frac{2\Delta(n, \delta)}{\Gamma_f}
\end{equation*}
\end{lemma}
\begin{proof}
We can then write:
\begin{align*}
    & \EE_{P_f}\left[\one\{\hat{\phi}(x_1) = \hat{\phi}(x_2)\}\TV{f^\star(\cdot \mid x_1, x', t, h) - f^\star(\cdot \mid x_2, x', t, h)}\right] \\
    &\le \EE_{P_f}\left[\one\{\hat{\phi}(x_1) = \hat{\phi}(x_2)\}\TV{f^\star(\cdot \mid x_1, x', t, h) - \hat{f}(\cdot \mid x_1, x', t, h)}\right] \\
    &+ \EE_{P_f}\left[\one\{\hat{\phi}(x_1) = \hat{\phi}(x_2)\}\TV{\hat{f}(\cdot \mid x_1, x', t, h) - f^\star(\cdot \mid x_2, x', t, h)}\right]
\end{align*}

We bound the two terms on the right hand side as following. First term is bounded as:
\begin{align*}
    &\EE_{(t, h, x_1, x_2, x') \sim P_f}\left[\one\{\hat{\phi}(x_1) = \hat{\phi}(x_2)\}\TV{f^\star(\cdot \mid x_1, x', t, h) - \hat{f}(\cdot \mid x_1, x', t, h)}\right] \\
    &\le \EE_{(t, h, x_1, x_2, x') \sim P_f}\left[\TV{f^\star(\cdot \mid x_1, x', t, h) - \hat{f}(\cdot \mid x_1, x', t, h)}\right]\\
    &= \EE_{(t, h, x_1, x_2, x') \sim D}\left[\TV{f^\star(\cdot \mid x_1, x', t, h) - \hat{f}(\cdot \mid x_1, x', t, h)}\right] \le \Delta(n, \delta).
\end{align*}

The second term is bounded as:
\begin{align*}
    &\EE_{(t, h, x_1, x_2, x') \sim P_f}\left[\one\{\hat{\phi}(x_1) = \hat{\phi}(x_2)\}\TV{\hat{f}(\cdot \mid x_1, x', t, h) - f^\star(\cdot \mid x_2, x', t, h)}\right]\\
    &=\EE_{(t, h, x_1, x_2, x') \sim P_f}\left[\one\{\hat{\phi}(x_1) = \hat{\phi}(x_2)\}\TV{\hat{f}(\cdot \mid x_2, x', t, h) - f^\star(\cdot \mid x_2, x', t, h)}\right]\\
    &\le \EE_{(t, h, x_1, x_2, x') \sim P_f}\left[\TV{\hat{f}(\cdot \mid x_2, x', t, h) - f^\star(\cdot \mid x_2, x', t, h)}\right]\\
    &= \EE_{(t, h, x_2, x') \sim D}\left[\TV{\hat{f}(\cdot \mid x_2, x', t, h) - f^\star(\cdot \mid x_2, x', t, h)}\right] \le \Delta(n, \delta).
\end{align*}
Adding these two upper bounds and triangle inequality, we get:
\begin{equation*}
    \EE_{P_f}\left[\one\{\hat{\phi}(x_1) = \hat{\phi}(x_2)\}\TV{f^\star(\cdot \mid x_1, x', t, h) - f^\star(\cdot \mid x_2, x', t, h)}\right] \le 2 \Delta(n, \delta).
\end{equation*}

We define a shorthand:
\begin{equation}
\Ecal(s, \stil, t, h) = \EE_{x \sim q(\cdot \mid s, \xi), \xtil \sim q(\cdot \mid \stil, \xitil), (\xi, \xitil, \xi') \sim P_f(\cdot, \cdot, \cdot \mid t, h)}\left[\one\{\hat{\phi}(x) = \hat{\phi}(\xtil)\}\right],
\end{equation}
using which we lower bound the left hand side as follows:
\begin{align*}
   &\EE_{(t, h, x, \xtil, x') \sim P_f}\left[\one\{\hat{\phi}(x) = \hat{\phi}(\xtil)\}\TV{f^\star(\cdot \mid x, x', t, h) - f^\star(\cdot \mid \xtil, x', t, h)}\right] \\
   &= \sum_{s, \stil \in \Scal}  
   \sum_{1 \le t < h \le H+1} \Ecal(s, \stil, t, h)\sum_{s' \in \Scal} P_f(t, h, s, \stil, s') \TV{f^\star(\cdot \mid s, s', t, h) - f^\star(\cdot \mid \stil, s', t, h)} \\
   &= \sum_{s, \stil \in \Scal, s \ne \stil}  
   \sum_{1 \le t < h \le H+1} \Ecal(s, \stil, t, h)\sum_{s' \in \Scal} P_f(t, h, s, \stil, s') \TV{f^\star(\cdot \mid s, s', t, h) - f^\star(\cdot \mid \stil, s', t, h)} \\
   &\ge \min_{s, \stil, s \ne \stil, t, h} \Ecal(s, \stil, t, h) \Gamma_f.
\end{align*}
Combining the lower bound and upper bound completes the proof.
\end{proof}
\textcolor{red}{YE:why the second relation holds?}


We can prove a similar result for backward coupling distribution.
\begin{lemma} Fix $\delta \in (0, 1)$. Given $\hat{f} = \hat{p}, \hat{\phi}$ as the ERM solution with $n$ samples, we have with probability at least $1-\delta$:
\begin{equation*}
    \EE_{P_b}\left[\one\{\hat{\phi}(x') = \hat{\phi}(
    \xtil')\}\TV{f^\star(\cdot \mid x, x', t, h) - f^\star(\cdot \mid x, \xtil', t, h)}\right] \le 2 \Delta(n, \delta).
\end{equation*}
\end{lemma}
\begin{proof}
We can then write:
\begin{align*}
    & \EE_{P_b}\left[\one\{\hat{\phi}(x') = \hat{\phi}(\xtil')\}\TV{f^\star(\cdot \mid x, x', t, h) - f^\star(\cdot \mid x, \xtil', t, h)}\right] \\
    &\le \EE_{P_b}\left[\one\{\hat{\phi}(x') = \hat{\phi}(\xtil')\}\TV{f^\star(\cdot \mid x, x', t, h) - \hat{f}(\cdot \mid x, \xtil', t, h)}\right] \\
    &+ \EE_{P_b}\left[\one\{\hat{\phi}(x') = \hat{\phi}(\xtil')\}\TV{\hat{f}(\cdot \mid x, x', t, h) - f^\star(\cdot \mid x, \xtil', t, h)}\right]
\end{align*}

We bound the two terms on the right hand side as following. First term is bounded as:
\begin{align*}
    &\EE_{(t, h, x, x', \xtil') \sim P_b}\left[\one\{\hat{\phi}(x') = \hat{\phi}(\xtil')\}\TV{f^\star(\cdot \mid x, x', t, h) - \hat{f}(\cdot \mid x, \xtil', t, h)}\right] \\
    &\le \EE_{(t, h, x, x', \xtil') \sim P_b}\left[\TV{f^\star(\cdot \mid x, x', t, h) - \hat{f}(\cdot \mid x, \xtil', t, h)}\right]\\
    &= \EE_{(t, h, x, x') \sim D}\left[\TV{f^\star(\cdot \mid x, x', t, h) - \hat{f}(\cdot \mid x, x', t, h)}\right] \le \Delta(n, \delta).
\end{align*}

The second term is bounded as:
\begin{align*}
    &\EE_{(t, h, x, x', \xtil') \sim P_b}\left[\one\{\hat{\phi}(x') = \hat{\phi}(\xtil')\}\TV{\hat{f}(\cdot \mid x, x', t, h) - f^\star(\cdot \mid x, \xtil', t, h)}\right] \\
    &=\EE_{(t, h, x, x', \xtil') \sim P_b}\left[\one\{\hat{\phi}(x') = \hat{\phi}(\xtil')\}\TV{\hat{f}(\cdot \mid x, \xtil', t, h) - f^\star(\cdot \mid x, \xtil', t, h)}\right] \\
    &\le \EE_{(t, h, x, x', \xtil') \sim P_b}\left[\TV{\hat{f}(\cdot \mid x, \xtil', t, h) - f^\star(\cdot \mid x, \xtil', t, h)}\right]\\
    &= \EE_{(t, h, x, x') \sim D}\left[\TV{\hat{f}(\cdot \mid x, x', t, h) - f^\star(\cdot \mid x, x', t, h)}\right] \le \Delta(n, \delta).
\end{align*}
Adding these two upper bounds and triangle inequality, gives us the result.
\end{proof}

==> notation.tex <==
%auto-ignore

\newcommand{\sd}{s}
% \newcommand{\se}{e}
\newcommand{\sx}{\xi}
\newcommand{\sdh}[1][h]{\sd_{#1}}
\newcommand{\sxh}[1][h]{\sx_{#1}}
% \newcommand{\seh}[1][h]{\se_{#1}}

\newcommand{\Sf}{\mathcal{Z}}
\newcommand{\Sfcard}{Z}
\newcommand{\Sfh}[1][h]{\Sf_{#1}}
\newcommand{\sff}{z}
\newcommand{\sfh}[1][h]{\sff_{#1}}

\newcommand{\Sd}{\mathcal{S}}
\newcommand{\Sdcard}{S}
\newcommand{\Sdh}[1][h]{\Sd_{#1}}

\newcommand{\Sx}{\Xi}
\newcommand{\Sxh}[1][h]{\Sx_{#1}}
\newcommand{\Sxcard}{|\Xi|}

\newcommand{\PiEnd}{\Pi_d}

\newcommand{\pt}{\upsilon}
\newcommand{\pts}{\Upsilon}

\newcommand{\mapping}{\varphi}

\newcommand{\open}{\Pi_{\circ}}
\newcommand{\policies}{\Pi}
\newcommand{\nspolicies}{\Pi_{\textrm{NS}}}

\newcommand{\todo}{\textcolor{red}}
\newcommand{\emf}{q}
\newcommand{\hatp}{\hat{\phi}}
\newcommand{\etamin}{\eta_{min}}
\newcommand{\hatpi}{\hat{\pi}}
\newcommand{\Deltaind}[1]{\Delta_{#1}}
\newcommand{\Deltapol}{\Delta^{\textrm{pol}}}
\newcommand{\Deltareg}{\Delta_{\textrm{reg}}}
\newcommand{\step}{\tau}
\newcommand{\supp}{\textrm{supp}}
\newcommand{\TV}[1]{\left\|#1\right\|_{\textrm{TV}}}
\newcommand{\dcoup}{D_{\textrm{coup}}}
\newcommand{\dcoupi}{D^{(i)}_{\textrm{coup}}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\hatpc}{\hat{\phi}^\circ}

\newcommand{\ps}{\phi^\star_z}
\newcommand{\edo}{\phi^\star}
\newcommand{\exo}{\phi^\star_{\xi}}

\newcommand{\hatedo}{\hat{\phi}}
\newcommand{\hatexo}{\hat{\phi}_{\xi}}

\newcommand{\hatedoh}{\hat{\phi}_{h}}
\newcommand{\hatexoh}{\hat{\phi}_{\xi,h}}

\newcommand{\new}[1]{\textcolor{blue}{#1}}
\newcommand{\newest}[1]{\textcolor{red}{#1}}

%\newcommand{\ps}{\phi^\star}
%\newcommand{\pe}{\phi^\star_e}
%\newcommand{\pg}{\phi^\star_g}
%\newcommand{\hatpe}{{\widehat{\phi}}_e}
%\newcommand{\hatpeh}[1]{{\widehat{\phi}}_{e,#1}}

%\newcommand{\pd}{\phi^\star_d}
%\newcommand{\px}{\phi^\star_x}

\renewcommand{\hatp}{\hat{\phi}}
\newcommand{\hatS}{\widehat{\Scal}}
\newcommand{\hatw}{\hat{w}}
\newcommand{\unf}{{\tt Unf}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\Range}{{\tt Range}}
\newcommand{\PSDP}{{\tt PSDP}\xspace}
\newcommand{\VI}{{\tt VI}\xspace}
\newtheorem{assumption}{Assumption}

% Algorithm related macros
% \newcommand{\algname}{{\tt GenIK}\xspace}
% \newcommand{\algppe}{{\tt PPE}\xspace}
% \newcommand{\algppelong}{Path Prediction and Elimination\xspace}
\newcommand{\algppe}{{\tt PPE}\xspace}
\newcommand{\algppelong}{Predictive Path Elimination \xspace}
\newcommand{\mycomment}[1]{\hfill\textcolor{blue}{//#1}}


==> sections/intro.tex <==
%auto-ignore

\section{Introduction}
% This section written by LM, 04/02

\textit{Problem Motivation}: Consider multiple collaborative robots (cobots) in an industrial assembly setting, tasked with improving objects' manipulation (for example, on a moving conveyor belt) efficiency alongside human warehouse workers.  These cobots must cooperatively coordinate their actions in a ``safety-preserving" manner so that humans are not injured. Suppose that arrays of RGB+Depth cameras feed situational awareness to a motion planning algorithm that controls these cobots.  %The  control behavior of human workers may cover a wide policy class range (given that different human beings may have different preferences for executing pick-and-place actions).
Traditionally, in such a control system, the description of the dynamic evolution of the overall system behavior is called a state. Suppose the robots are anthropomorphic arms, the state for each robot in the cobot would consist of seven numbers -- one for each joint angle that dictates the motion between robot links, which is the \textit{set of numbers from which the entire future of behavior of the system may be solved, provided that the future inputs to the system are known}~\cite{Kalman1958}. 

The properties of the cobots, where the behavior of the overall system in closed-loop becomes difficult to analyze by aggregating the individual states of each open-loop robot in an an open-loop (or even closed-loop) fashion becomes difficult to analyze when perception, sensing, control and the software must be ``tightly" integrated to provide a consistent operation in the face of parametric and non-parametric uncertainties, environmental disturbance, model mismatch between the real-world and its (mathematical) representation e.t.c. 

In this work, we introduce the notion of an all-encompassing ``latent state" of the system that captures not just the internal, or endogenous, state of each agent acting alone in a \textit{complex system}, but rather encapsulates the overall system dynamics that may affect the evolution of the complex system as a whole. This latent state is a composition of the endogenous state together with the system's exogenous state. To ``discover" this latent state in a principled computational learning framework, we will be leveraging 
%
\begin{inparaenum}[(a)]
  \item deep learning as a universal function approximation tool; ; and 
  \item the principles of dynamic programming and optimality~\cite{Bellman1957, Bellman1962}.
 \end{inparaenum}

The algorithm which accomplishes this latent state discovery is termed ``Genik". Genik uses a generalized inverse model (predicting control laws from distant observations) with an information bottleneck on the representations of the complex system.  We shall  demonstrate Genik on a system with multiple agents viz.,  
\begin{inparaenum}[(i)]
  \item navigation in a simulated maze from high-resolution images; and
  %
  \item control of a seven degrees-of-freedom (DOF) robot from the images of the environment in the presence of a distracting video in the background.
\end{inparaenum}  

This problem study is motivated by robotic applications, including warehouse pick-and-place automation tasks, dynamic navigation in a complex state space, optimal path planning, and complex systems analysis. For example, in the path planning of multiple collaborative robots that must navigate a warehouse fulfillment center, arranging movable totes, picking up shelves from one location to another for human packaging operators in order to assure efficiency in the internal logistics operations
of a plant. In pick-and-place of objects within plastic totes, a robot must discover the specific object to be picked, while working alongside human packaging operators who share the complete workspace volume with the robot. 

\textit{Literature Review}:

==> sections/jl_abstract.tex <==
%auto-ignore


\abstract{A person walking along a city street who tries to model all aspects of the world would quickly be overwhelmed by a multitude of shops, cars, and people moving in and out of view, following their own complex and inscrutable dynamics.  Exploration and navigation in such an environment is an everyday task, requiring no vast exertion of mental resources.  Is it possible to turn this fire hose of sensory information into a minimal latent state which is necessary and sufficient for an agent to successfully act in the world? We formulate this question concretely, and propose the Agent-Controllable State Discovery algorithm ($\selfstate$), which has theoretical guarantees and is practically demonstrated to discover the \textit{minimal controllable latent state} which contains all of the information necessary for controlling the agent, while fully discarding all irrelevant information.    This algorithm consists of a multi-step inverse model (predicting actions from distant observations) with an information bottleneck.  \selfstate enables localization, exploration, and navigation without reward or demonstrations.  We demonstrate the discovery of controllable latent state in three domains: localizing a robot arm with distractions (e.g., changing lighting conditions and background), exploring in a maze alongside other agents, and navigating in the Matterport house simulator.}


% \abstract{A person walking along a city street who tries to model all aspects of the world would quickly be overwhelmed by a multitude of shops, cars, and people moving in and out of view, following their own complex and inscrutable dynamics.  Exploration and navigation in such an environment is an everyday task, requiring no vast exertion of mental resources.  Is it possible to turn this fire hose of sensory information into a minimal latent state which is necessary and sufficient for an agent to successfully act in the world? We formulate this question concretely, and propose the Agent-Controllable State Discovery algorithm ($\selfstate$), which has theoretical guarantees and is practically demonstrated to discover the \textit{minimal controllable latent state} which contains all of the information necessary for controlling the agent, while fully discarding all irrelevant information.    This algorithm consists of a multi-step inverse model (predicting actions from distant observations) with an information bottleneck.  \selfstate enables localization, exploration, and navigation without reward or demonstrations.  We test the efficacy of our propositions and theory %discovery of controllable latent state 
% in three domains namely,
% %
% \begin{inparaenum}[(a)]
% \item localizing a robot arm with distractions (e.g., changing lighting conditions and background);
%  \item exploring in a maze alongside other agents; and
%  \item navigating in the Matterport house simulator.
%  \end{inparaenum}
%  In all, our experiments confirm our theoretical formalisms and guarantees.
%  }


==> sections/lm_abstract.tex <==
%auto-ignore

\begin{sciabstract}
Informed by the growing availability of richly-available multimodal sensory information in emerging exploratory tasks for complex systems such as multi-agent control and reinforcement learning, and the efficacy of deep learning to reason over such sensor inputs, the concept of  ``state" and ``transition matrix" as originally conceived by R.E. Kalman et al is revisited. Introducing the concept of a ``latent state", we propose a simple and generic algorithm: ``Genik"; Genik  can be solved via the principle of optimality and dynamic programming -- over a purely random policy without need for reward, or programming by demonstration, for example. We build upon the recent results from our group, and posit that a complex systems' latent states be ``discovered" using generalized performance indexes over sensor representations to optimize for classes of input signals that assure ``optimality" of the designed system. %Given the efficiency of our general purpose approach, and the emerging need to process large amounts of information, the techniques proposed here may become widely useful in the future.
\end{sciabstract}

==> tech_report/math_commands.tex <==
%auto-ignore

%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
% \DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
% \SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

